Ninety-Six Ways to Measure a Scribe: Fragmented Evaluation of Ambient Scribes in Healthcare

Ambient artificial intelligence (AI) scribes have moved rapidly from experimental pilots to enterprise-wide deployment across health systems, promising reduced documentation burden and improved clinician experience. While research evaluating these tools has expanded quickly, there are no agreed-upon protocols or standardized metrics for assessing their performance, making it difficult to compare findings or cumulatively synthesize evidence across studies. Across 54 recent evaluation studies, we identify ten evaluation dimensions and 40 distinct metrics, operationalized in 96 different ways-35 of them (36%) used by only a single study. Assessment is dominated by documentation efficiency and time, measured in 44 of 54 studies. The other dimensions appear at broadly similar rates (16-24 studies each), and safety and clinical outcome least consistently of all. Ripple effects on the broader care system, such as impact on patients' care outcomes, redistribution of work, changes in billing and coding intensity, and downstream use of notes by other clinicians are rarely assessed. Moreover, the metrics used rely heavily on self-report and are fragmented and inconsistently operationalized, which limits comparability and hinders synthesis across studies. As an effort to support more rigorous and cumulative evaluation, in this paper we review the study designs, data sources, and metrics commonly used to evaluate ambient AI scribes in healthcare settings, discuss the limitations of current evaluation practice, and argue for a more holistic approach grounded in a standardized, multi-dimensional set of metrics.

==> details_table.tex <==
% Study-characteristics table. Requires longtable, booktabs, array, natbib.
\begingroup
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.25}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\begin{longtable}{@{}L{2.0cm} L{2.15cm} L{1.4cm} L{2.85cm} L{3.35cm} L{2.75cm}@{}}
\caption{Characteristics of the 39 reviewed studies, emphasizing study type, methodology, and data type. Departments and durations are given for context. ``EHR analytics'' denotes vendor/Epic Signal-type audit-log metrics.}\label{tab:studies}\\
\toprule
\textbf{Study} & \textbf{Dept.\ / setting} & \textbf{Duration} & \textbf{Study type} & \textbf{Methodology} & \textbf{Data type \& amount} \\
\midrule
\endfirsthead
\multicolumn{6}{@{}l}{\scriptsize\emph{Table~\ref{tab:studies} continued from previous page}}\\
\toprule
\textbf{Study} & \textbf{Dept.\ / setting} & \textbf{Duration} & \textbf{Study type} & \textbf{Methodology} & \textbf{Data type \& amount} \\
\midrule
\endhead
\midrule\multicolumn{6}{r@{}}{\scriptsize\emph{continued on next page}}\\ \endfoot
\bottomrule\endlastfoot
\citet{ballantyne2025using} & Primary care (NZ) & survey window & Qualitative exploratory & Anonymous cross-sectional survey & 197 clinician surveys \\\addlinespace[1pt]
\citet{rotenstein2026changes} & Ambulatory (multisite) & 2 yr & Multisite longitudinal observational cohort & EHR (Epic Signal) analytics & 181,273 encounters \\\addlinespace[1pt]
\citet{toussi2026impact} & Oncology, primary care & 4 mo & Two-phase mixed-design pilot & Pre/post surveys + billing/coding data & 25 physicians; 35 surveys; billing data \\\addlinespace[1pt]
\citet{nguyen2023implementing} & Cancer care & 1 mo & Mixed-methods longitudinal pilot & Validated scales + semi-structured interviews & 21 participants; 8 interviews \\\addlinespace[1pt]
\citet{haberle2024impact} & Multispecialty (adult/peds) & 7 mo & Peer-matched controlled cohort & EHR history + post-surveys + operational/LTR reports & 35,000+ DAX encounters \\\addlinespace[1pt]
\citet{rui2025qualitative} & Multispecialty (2 systems) & $\sim$3 mo & Mixed-methods (survey + open-ended) & Pre/during/post surveys & 155 clinician surveys \\\addlinespace[1pt]
\citet{adler2026subjective} & Medicine (ambulatory, academic) & 12-wk pre/post & Retrospective observational & Survey + EHR measures + regression & 310 physicians; 252 surveys \\\addlinespace[1pt]
\citet{shin2025influence} & Pediatrics & 3 mo & Single-center randomized QI trial & Pre/post; Epic Signal + wRVU data & 2,064 encounters; 17 KLAS surveys \\\addlinespace[1pt]
\citet{holmgren2026ambient} & Ambulatory (enterprise) & $\sim$2 yr & Retrospective EHR analytics (diff-in-diff, event study) & EHR / claims / RVU analytics & 1.2M encounters \\\addlinespace[1pt]
\citet{patel2026effect} & Primary \& non-primary care & 3 mo & Cross-sectional observational survey & Patient survey & 8,120 patient surveys \\\addlinespace[1pt]
\citet{schneider2026impact} & Multispecialty (mostly primary care) & 8 mo & QI pilot survey & Pre/post surveys & 541 surveys (329 + 212) \\\addlinespace[1pt]
\citet{mccrudden2026ai} & Mental health & 1 yr & Retrospective observational mixed-methods & Note-quality, use \& productivity analytics + open-ended surveys & 286,911 notes; 121 surveys \\\addlinespace[1pt]
\citet{shah2025ambient} & Primary \& ambulatory care & 4 mo & Prospective QI pilot & Pre/post surveys & 76 survey responses \\\addlinespace[1pt]
\citet{moura2026hybrid} & Primary care & 4 mo & Retrospective cohort (stepped-wedge) & EHR Signal + data-warehouse analytics (GEE) & 108,224 encounters \\\addlinespace[1pt]
\citet{north2025ambient} & Primary care (org-wide) & $\sim$1 yr & Retrospective pre/post observational & EHR analytics & 22,495 physician-weeks; 582 physicians \\\addlinespace[1pt]
\citet{guo2025ambient} & Primary care \& others & 6 mo (3 pre/3 post) & QI exploratory pilot & EHR analytics (pre/post) & 46 clinicians ($\geq$10 notes each) \\\addlinespace[1pt]
\citet{pelletier2025effect} & Pediatrics & 6 mo & Mixed-methods pilot & EHR analytics + provider \& caregiver surveys & 31,931 encounters; 132 surveys; 47 comments \\\addlinespace[1pt]
\citet{cao2024artificial} & Dermatology & 2 yr & Mixed-methods pilot & Pre/post productivity + note metrics + surveys & encounters + notes; 6 clinician, 23 patient surveys \\\addlinespace[1pt]
\citet{memon2026performance} & General medicine & 16 wk & Mixed-methods pilot & Staff/patient surveys, PDQI, ROUGE, EMR review, interviews & 7,499 consultations; 65 surveys; 18 PDQI / 21 ROUGE \\\addlinespace[1pt]
\citet{wright2025effect} & EM, IM, OB/GYN, Peds (trainees) & 2 mo & Prospective observational pilot & EHR (Epic Signal) analytics + pre/post surveys & 84 surveys; 31 Signal logs \\\addlinespace[1pt]
\citet{harvey2025ambient} & Ambulatory / surgery & 3 mo & Mixed-methods pilot (preliminary) & Pre/post surveys + Epic Signal + billing + patient satisfaction & 79 surveys; Signal from 3 surgeons \\\addlinespace[1pt]
\citet{evans2025impact} & Allied health (multi-institution) & baseline + 6 wk + 3 mo & Mixed-methods implementation & Clinician \& patient surveys + productivity + interviews & 119 clinician + 157 patient surveys \\\addlinespace[1pt]
\citet{baldwin2025ambient} & Oncology & 4 mo & Prospective pilot & Utilization analytics + surveys + interviews & 722 encounters (620 analyzed) \\\addlinespace[1pt]
\citet{rabbani2025ambient} & Pediatric primary care & 12 wk & Mixed-methods pilot (pre/post) & EHR analytics + clinician \& patient surveys & 19,264 encounters; 39 clinician + $\sim$300 patient surveys \\\addlinespace[1pt]
\citet{castro2026psychiatric} & Primary care & 2 yr & Retrospective cohort (matched case-control) & Note-text analysis + PHQ-9 & 20,302 encounters / notes \\\addlinespace[1pt]
\citet{wright2026enterprise} & Ambulatory \& ED (enterprise) & 3 mo & Mixed-methods & Utilization data + post-use survey & 1,223 users; 209 surveys \\\addlinespace[1pt]
\citet{preiksaitis2026ambient} & Emergency medicine & 8 mo & Retrospective observational & EHR audit-log analytics & 8,740 encounters (976 AI-documented) \\\addlinespace[1pt]
\citet{alpert2025evaluating} & Primary care & 4 wk & Mixed-methods QI pilot & Pre/post EHR analytics + surveys + interviews & validated scales; 10 interviews \\\addlinespace[1pt]
\citet{van2026ambient} & General practice (multicentre) & $\sim$7 mo & Prospective multicentre before-after mixed-methods & EHR data (GLMM) + interviews & 535 observed consultations \\\addlinespace[1pt]
\citet{tierney2025ambient} & Multispecialty (MH, EM, primary care) & $\sim$1 yr & Retrospective commentary & Post-visit patient \& physician surveys + use data & 2.58M encounters; 102 physician + 118 patient responses \\\addlinespace[1pt]
\citet{pearlman2025use} & Ambulatory & 3 mo & Retrospective cohort & Pre/post propensity-score-weighted EHR analysis & Epic Signal EHR records \\\addlinespace[1pt]
\citet{lukac2025ambient} & Primary / medical / surgical & 3 mo & Three-group pragmatic RCT & Pre/post survey + Epic Signal EHR & $\sim$72,000 encounters (DAX / Nabla / control) \\\addlinespace[1pt]
\citet{waken2026longitudinal} & Primary care & 48 wk & Longitudinal quasi-experimental & Pre/post analysis & 314,845 encounters \\\addlinespace[1pt]
\citet{baldwin2025early} & Oncology & 4 mo & Prospective pilot & Surveys + interviews & 620 / 4,449 visits (14\%) \\\addlinespace[1pt]
\citet{olson2025use} & Ambulatory (MDs \& APPs) & 9 mo & Quality-improvement study & 30-day pre/post surveys & 263 survey responses \\\addlinespace[1pt]
\citet{tan2026impact} & Future Health System & 5 mo & Prospective observational time-motion & Matched design, time-motion observation + patient surveys & 169 observed consultations; 39 surveys \\\addlinespace[1pt]
\citet{marquis2026ai} & Emergency & 8 mo & Cross-sectional descriptive mixed-methods pilot & Cross-sectional survey (quant + free-text) & 14 survey respondents \\\addlinespace[1pt]
\citet{chowdhury2026comparing} & Outpatient (any specialty) & $\sim$2.5 mo (2$\times$1 mo) & Randomized crossover trial & Baseline + post-study surveys across 2 tools & 136 surveys \\\addlinespace[1pt]
\citet{duggan2024clinician} & Not specified & 7-wk pilot (5-wk use) & Prospective single-group pre/post QI & EHR analytics + surveys & Not specified \\\addlinespace[1pt]
\end{longtable}
\endgroup
